What is the nature of GW230529? An exploration of the gravitational lensing hypothesis

On the 29th of May 2023, the LIGO-Virgo-KAGRA Collaboration observed a compact binary coalescence event consistent with a neutron star-black hole merger, though the heavier object of mass 2.5-4.5 $M_\odot$ would fall into the purported lower mass gap. An alternative explanation for apparent observations of events in this mass range has been suggested as strongly gravitationally lensed binary neutron stars. In this scenario, magnification would lead to the source appearing closer and heavier than it really is. Here, we investigate the chances and possible consequences for the GW230529 event to be gravitationally lensed. We find this would require high magnifications and we obtain low rates for observing such an event, with a relative fraction of lensed versus unlensed observed events of $2 \times 10^{-3}$ at most. When comparing the lensed and unlensed hypotheses accounting for the latest rates and population model, we find a 1/58 chance of lensing, disfavoring this option. Moreover, when the magnification is assumed to be strong enough to bring the mass of the heavier binary component below the standard limits on neutron star masses, we find high probability for the lighter object to have a sub-solar mass, making the binary even more exotic than a mass-gap neutron star-black hole system. Even when the secondary is not sub-solar, its tidal deformability would likely be measurable, which is not the case for GW230529. Finally, we do not find evidence for extra lensing signatures such as the arrival of additional lensed images, type-II image dephasing, or microlensing. Therefore, we conclude it is unlikely for GW230529 to be a strongly gravitationally lensed binary neutron star signal.

==> tidal_compatibility.tex <==
As explained in~\citet{Pang:2020kle}, if an event is lensed, there would be a 
discrepency between the measured tidal deformability and the one expected from 
the delensed source-frame masses. Therefore, here, wecompare the tidal deformabilities
measured in~\citet{LIGOScientific:2024elc} for the runs done with the 
IMRPhenomPv2\_NRTidalv2 waveform~\citep{Dietrich:2019kaq} and the ones we would expect from 
the systems after we delens them. For the latter, we follow the steps described in 
Section~\ref{sec:delensing_effect} for the posteriors found when analyzing GW230529 with 
tidal effects. There are two different cases considered for the initial parameter estimation 
runs: one with a low-spin constraint on the secondary and one with a low-spin constraint for both 
objects. 

After the delensing is done, we calculate the tidal deformabilities for the two objects by 
using the maximum probability EoS from~\citet{Huth:2021bsp}, and use Eq.~\eqref{eq:lambda_tilde_def}
to find the distribution for $\tilde{\Lambda}$. 
This parameter is the best measured one 
in relation with the tidal deformabilities since it appears at the lowest PN order in the 
waveform~\citep{Hinderer:2009ca}. The left panel in Fig.~\ref{fig:tidal_comparisons} show the 
$\tilde{\Lambda}$ distributions found for the single low spin constrain for the various 
$m_1$ cuts overlaid with the value found in the original analysis. The right panel shows the same
for the double low spin constrain case. For the single low spin prior, 
the distributions 
found via delensing are relatively low, which comes from the higher masses expected for the 
lighest component in this case. The value that would be the most compatible is the one for 
the lowest heavier component mass, which is also the case giving the most unphysical 
scenario since the mass of the lighter object would have a large probability of being sub-solar.
Moreover, the distributions do not have shapes comparable with 
the one that is measured. For the double low spin case, the distributions are more peaked 
but fall in the lower density regions of the original $\tilde{\Lambda}$ distribution, which 
shows incompatibility between the two. The only exception is that of the highest mass for the 
heavier object where the distribution is close to the peak of the measured one.

\begin{figure*}
    \includegraphics[keepaspectratio, width=0.49\textwidth]{figures/tilde_lambda_low_spin.pdf}
    \includegraphics[keepaspectratio, width=0.49\textwidth]{figures/tilde_lambda_double_low_spin.pdf}
    \caption{Comparison between the tidal deformability distributions found by 
    delensed GW230529 and the measured ones. The left panel shows the results for the 
    low-spin constraint on the secondary, while the right panel shows the results for the 
    double low-spin constraint. The distributions are overlaid with the measured 
    $\tilde{\Lambda}$ values measured for each spin priors used when analyzing 
    the event with IMRPhenomPv2\_NRTidalv2. While there is some degree of overlap, the shape of the
    distributions are very different and there are also many regions without overlap. So, 
    the compatibility between the measured and 
    expected tidal deformabilities is low in all cases.}
    \label{fig:tidal_comparisons}
\end{figure*}

Once, the distributions for $\tilde{\Lambda}$ are build, we can 
quantify the compatibility between the two follow the posterior 
overlap approach explained in~\citet{Haris:2018vmn}. Therefore, 
we calculate
\begin{equation}
    \mathcal{O}_{\theta} = \int \mathrm{d}\theta \, \frac{p(\theta | d_{GW}) p(\theta | \mathrm{Delens})}{p(\theta)} \,,
\end{equation}
where $\theta$ is the parameter of interest, $d_{GW}$ is the measured data,
and $\mathrm{Delens}$ is the delensed data. The denominator corresponds to 
the prior distribution for the parameter. We then calculate the overlap 
statistic for $\LambdaTilde$ and $\Lambda_2$. The results are shown in 
Table~\ref{tab:po_lambdas}. None of them favors the 
lensing hypothesis, with, at best, am uninformative result, and, in most 
cases, a disfavoring of the lensing hypothesis. Thus, this test 
further stacks up evidence against the lensing hypothesis for GW230529.

\begin{table}
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        $m_1\,(M_{\odot})$ & $\log_{10}(\mathcal{O}_{\LambdaTilde})$ & $\log_{10}(\mathcal{O}_{\Lambda_{2}})$ \\
        \hline
        \hline 
        \multicolumn{3}{|c|}{High spin case} \\
        \hline
        1.76 & -0.32 & -0.60 \\
        1.99 & -0.22 & -0.40 \\
        2.28 & -0.25 & -0.23 \\
        2.50 & -0.35 & -0.13 \\
        \hline
        \hline 
        \multicolumn{3}{|c|}{Low spin case} \\
        \hline
        1.76 & -1.10 & -4.65 \\
        1.99 & -1.11 & -3.76 \\
        2.28 & -0.49 & -2.29 \\
        2.50 & 0.03 & -1.21 \\
        \hline
    \end{tabular}
    \caption{$\log_{10}$ posterior overlap statistic for the tidal deformability
    of the secondary object and $\LambdaTilde$. The highest value 
    found is uninformative, while all the others disfavor the lensing hypothesis,
    showing the incompatibility between the measured and expected tidal 
    deformabilities, should the event be lensed.}
    \label{tab:po_lambdas}
\end{table}

Going further, one can study if the high tidal deformability
that a lensed low-mass secondary would present
should have been observable in GW230529.
In a more general simulation study,
\citet{Golomb:2024mmt} found that if both components are neutron stars
and at least one is sub-solar,
this should be clearly measurable.
\dk{Justin's injection study would then logically continue this train of thought.}

